Robotic Wireless Sensor Networks

In this chapter, we present a literature survey of an emerging, cutting-edge, and multi-disciplinary field of research at the intersection of Robotics and Wireless Sensor Networks (WSN) which we refer to as Robotic Wireless Sensor Networks (RWSN). We define a RWSN as an autonomous networked multi-robot system that aims to achieve certain sensing goals while meeting and maintaining certain communication performance requirements, through cooperative control, learning and adaptation. While both of the component areas, i.e., Robotics and WSN, are very well-known and well-explored, there exist a whole set of new opportunities and research directions at the intersection of these two fields which are relatively or even completely unexplored. One such example would be the use of a set of robotic routers to set up a temporary communication path between a sender and a receiver that uses the controlled mobility to the advantage of packet routing. We find that there exist only a limited number of articles to be directly categorized as RWSN related works whereas there exist a range of articles in the robotics and the WSN literature that are also relevant to this new field of research. To connect the dots, we first identify the core problems and research trends related to RWSN such as connectivity, localization, routing, and robust flow of information. Next, we classify the existing research on RWSN as well as the relevant state-of-the-arts from robotics and WSN community according to the problems and trends identified in the first step. Lastly, we analyze what is missing in the existing literature, and identify topics that require more research attention in the future.

==> texfiles/sensing.tex <==
Since we are talking about Robotic wireless sensor network, the main focus
should be on multiple robots based sensing that involves realistic communication
constraints. 
While every function of a multi-robot system involves some sort of sensing
such as sensing RSSI, SINR, or locations of other nodes, in this section we
focus on works related to any kind of sensing in general. In this context, there
exist many work in the field of mobile sensor networks and distributed robotics
on coverage control, cooperative sensing. However as explained earlier, all
these works have some idealistic assumption about either communication or
control. So, in this section we only focus on works that involves realistic
models for both communication and control.

In the field of multi-agent sensing, distributed coverage of the area of
interest is a very well known field of research in the contexts of both Wireless
Sensor Network~\cite{wang2010coverage} and multi-robot systems~\cite
{cortes2004coverage}. In the contexts of WSN, coverage control algorithms focus
on the placements of mostly static sensor nodes to optimally cover the area of
interest. We do not present a survey of this well studied problem. An interested
reader is referred to a survey such as \cite{wang2010coverage}. However,
most of these works does not focus on using controlled mobility of the robots to
the advantage. On the other hand, there exist a class of coverage control
related articles in the field of coordinated robotic which focus on mostly the
control and path planning of the robots and graph point of view of
coverage problem by employing Voronoi partitions. However, these works does not
address the problem of collecting and communicating the sensed data effectively.
Only recently a small group of researchers started to look into multi-robot
sensing problem from both control and communication point of view. The work of
Kantaros and Zavlanos is mentionable in this context~\cite
{kantaros2014communication}. They looked into the coverage problem of multiple
robotic sensor placement by formulating a placement optimization problem
that takes into account realistic communication constraints as well as sensing
efficiencies of the robotic nodes. 
In \cite{yan2013communication}, Yan and Mostofi looked into the problem of
robotic path planning and optimal communication strategies in the context of a
single robot assisted sensing and data collections. 
Similar combined path planning and communication optimization in the
contexts of multiple robot based system is presented in the works of Ghaffarkhah
and Mostofi~\cite{ghaffarkhah2012optimal,ghaffarkhah2012path}. 
The works of Mostofi \et \cite{gonzalez2013cooperative,gonzalez2014integrated,mostofi2013cooperative} on
cooperative sensing and structure mapping are also related to this context.
In these works, the authors have leveraged pairs of coordinated robots and their RF communication abilities to sense/map unknown structures. They also
employed the concepts of compressible sampling/sensing~\cite
{candes2006compressive} and the well known RF communication properties
such as path loss and fading~\cite{rappaport1996wireless}.
The work by Le Ny, Ribeiro, and Pappas~\cite{le2012adaptive} also presents
optimization problem that couples motion planning and communication objective for
sensing. The work of Williams and Sukhatme~\cite{williams2011cooperative}
on multiple robot based plume detection, and Jiang and Zefran~\cite
{jiang2013coverage} on coverage control are also mentionable in this
context.
